DiffFace: Diffusion-based Face Swapping with Facial Guidance

In this paper, we propose a diffusion-based face swapping framework for the first time, called DiffFace, composed of training ID conditional DDPM, sampling with facial guidance, and a target-preserving blending. In specific, in the training process, the ID conditional DDPM is trained to generate face images with the desired identity. In the sampling process, we use the off-the-shelf facial expert models to make the model transfer source identity while preserving target attributes faithfully. During this process, to preserve the background of the target image and obtain the desired face swapping result, we additionally propose a target-preserving blending strategy. It helps our model to keep the attributes of the target face from noise while transferring the source facial identity. In addition, without any re-training, our model can flexibly apply additional facial guidance and adaptively control the ID-attributes trade-off to achieve the desired results. To the best of our knowledge, this is the first approach that applies the diffusion model in face swapping task. Compared with previous GAN-based approaches, by taking advantage of the diffusion model for the face swapping task, DiffFace achieves better benefits such as training stability, high fidelity, diversity of the samples, and controllability. Extensive experiments show that our DiffFace is comparable or superior to the state-of-the-art methods on several standard face swapping benchmarks.

==> figures/figures.tex <==
\newcommand{\figarch}{
\begin{figure*}[t]
\vspace{-5mm}
\centering
\includegraphics[width=1.0\linewidth]{figures/2.method/model_overview.pdf}\\
\makebox[0.25\linewidth][c]{\footnotesize{(a) Generator}}\hfill
\makebox[0.25\linewidth][c]{\footnotesize{(b) Mapping network}}\hfill
\makebox[0.25\linewidth][c]{\footnotesize{(c) Style encoder}}\hfill
\makebox[0.25\linewidth][c]{\footnotesize{(d) Discriminator}}\hfill \\
\vspace{1.9mm}
\caption{Overview of \stargan, consisting of four modules.
\textbf{(a)} The generator translates an input image into an output image
reflecting the domain-specific style code. \textbf{(b)} The mapping network transforms a latent code into style codes for multiple domains, one of which is randomly selected during training. \textbf{(c)} The style encoder extracts the style code of an image, allowing the generator to perform reference-guided image synthesis. \textbf{(d)} The discriminator distinguishes between real and fake images from multiple domains. Note that all modules except the generator contain multiple output branches, one of which is selected when training the corresponding domain.} 
\label{fig:networks}
\vspace{-2mm}
\end{figure*}
}


\newcommand{\figablation}{
\renewcommand{\h}{41mm}
\begin{figure}[t]
\vspace{-2mm}
\includegraphics[width=\h]{figures/3.1.ablation/config_abc.pdf}\hspace{-0.1mm}
\includegraphics[width=\h]{figures/3.1.ablation/config_d.pdf}\vspace{0.4mm}\\
\includegraphics[width=\h]{figures/3.1.ablation/config_e.pdf}\hspace{-0.1mm}
\includegraphics[width=\h]{figures/3.1.ablation/config_f.pdf}\\
\vspace{-3mm}
\caption{Visual comparison of generated images using each configuration in \Tref{tab:ablation}. Note that given a source image, the configurations (\arch{a}) - (\arch{c}) provide a single output, while (\arch{d}) - (\arch{f}) generate multiple output images.}\vspace{-3mm}
\label{fig:ablation}
\end{figure}
}


\newcommand{\figrefceleba}{
\begin{figure*}[t]
\centering
\begin{minipage}[c]{0.972\linewidth}
\includegraphics[width=1.0\linewidth]{figures/3.1.ref_guided/ref_celeba.pdf}\\
\vspace{-1mm}
\end{minipage}
\caption{Reference-guided image synthesis results on CelebA-HQ. 
The source and reference images in the first row and the first column are real images, while the rest are images generated by our proposed model, \stargan. Our model learns to transform a source image reflecting the style of a given reference image. High-level semantics such as hairstyle, makeup, beard and age are followed from the reference images, while the pose and identity of the source images are preserved. Note that the images in each column share a single identity with different styles, and those in each row share a style with different identities. 
}
\label{fig:refceleba}
\vspace{-1mm}
\end{figure*}
}


\newcommand{\figrandom}{
\renewcommand{\h}{17.0mm}
\newcommand{\hdataset}{1mm}
\newcommand{\hsrc}{0.5mm}
\newcommand{\himg}{-0.6mm}
\begin{figure*}[t]
\vspace{-10mm}
\footnotesize{
\makebox[\h][c]{\textbf{Source}}\hspace{\hsrc}
\makebox[\h][c]{MUNIT~\cite{huang2018munit}}\hspace{\himg}
\makebox[\h][c]{DRIT~\cite{lee2018drit}}\hspace{\himg}
\makebox[\h][c]{MSGAN~\cite{mao2019msgan}}\hspace{\himg}
\makebox[\h][c]{\textbf{Ours}}\hspace{\hdataset}
\makebox[\h][c]{\textbf{Source}}\hspace{\hsrc}
\makebox[\h][c]{MUNIT~\cite{huang2018munit}}\hspace{\himg}
\makebox[\h][c]{DRIT~\cite{lee2018drit}}\hspace{\himg}
\makebox[\h][c]{MSGAN~\cite{mao2019msgan}}\hspace{\himg}
\makebox[\h][c]{\textbf{Ours}}\vspace{0.1mm}
}\\\
\renewcommand{\himg}{-1mm}
\includegraphics[width=\h]{figures/3.2.latent_comparison/0.jpg}\hspace{\hsrc}
\includegraphics[width=\h]{figures/3.2.latent_comparison/1.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.latent_comparison/2.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.latent_comparison/3.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.latent_comparison/4.jpg}\hspace{\hdataset}
\includegraphics[width=\h]{figures/3.2.latent_comparison/5.jpg}\hspace{\hsrc}
\includegraphics[width=\h]{figures/3.2.latent_comparison/6.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.latent_comparison/7.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.latent_comparison/8.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.latent_comparison/9.jpg}\vspace{0.5mm}
\makebox[0.5\linewidth][c]{\footnotesize{(a) Latent-guided synthesis on CelebA-HQ}}\hfill
\makebox[0.5\linewidth][c]{\footnotesize{(b) Latent-guided synthesis on AFHQ}}\hfill
\vspace{1mm}
\caption{Qualitative comparison of latent-guided image synthesis results on the CelebA-HQ and AFHQ datasets. Each method translates the source images (left-most column) to target domains using randomly sampled latent codes. \textbf{(a)} The top three rows correspond to the results of converting male to female and vice versa in the bottom three rows. \textbf{(b)} Every two rows from the top show the synthesized images in the following order: cat-to-dog, dog-to-wildlife, and wildlife-to-cat.}
\vspace{-2mm}
\label{fig:latentguided}
\end{figure*}
}


\newcommand{\figref}{
\renewcommand{\h}{17mm}
\renewcommand{\hdataset}{1mm}
\renewcommand{\href}{0.5mm}
\renewcommand{\himg}{-0.7mm}
\begin{figure*}[t]
\vspace{-3mm}
\footnotesize{
\makebox[\h][c]{\textbf{Source}}\hspace{\himg}
\makebox[\h][c]{\textbf{Reference}}\hspace{\href}
\makebox[\h][c]{DRIT~\cite{lee2018drit}}\hspace{\himg}
\makebox[\h][c]{MSGAN~\cite{mao2019msgan}}\hspace{\himg}
\makebox[\h][c]{\textbf{Ours}}\hspace{\hdataset}
\makebox[\h][c]{\textbf{Source}}\hspace{\himg}
\makebox[\h][c]{\textbf{Reference}}\hspace{\href}
\makebox[\h][c]{DRIT~\cite{lee2018drit}}\hspace{\himg}
\makebox[\h][c]{MSGAN~\cite{mao2019msgan}}\hspace{\himg}
\makebox[\h][c]{\textbf{Ours}}\vspace{0.1mm}
}\\\
\renewcommand{\himg}{-1mm}
\includegraphics[width=\h]{figures/3.2.ref_comparison/0.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.ref_comparison/1.jpg}\hspace{\href}
\includegraphics[width=\h]{figures/3.2.ref_comparison/2.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.ref_comparison/3.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.ref_comparison/4.jpg}\hspace{\hdataset}
\includegraphics[width=\h]{figures/3.2.ref_comparison/5.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.ref_comparison/6.jpg}\hspace{\href}
\includegraphics[width=\h]{figures/3.2.ref_comparison/7.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.ref_comparison/8.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/3.2.ref_comparison/9.jpg}\vspace{0.5mm}
\makebox[0.5\linewidth][c]{\footnotesize{(a) Reference-guided synthesis on CelebA-HQ}}\hfill
\makebox[0.5\linewidth][c]{\footnotesize{(b) Reference-guided synthesis on AFHQ}}\hfill
\vspace{0.5mm}
\caption{Qualitative comparison of reference-guided image synthesis results on the CelebA-HQ and AFHQ datasets. Each method translates the source images into target domains, reflecting the styles of the reference images.}
\label{fig:refcompare}
\end{figure*}
}


\newcommand{\figffhq}{
\renewcommand{\h}{27.0mm}
\renewcommand{\himg}{-0mm}
\begin{figure}[t]
\vspace{-11mm}
\makebox[\h][c]{Source}\hspace{\himg}
\makebox[\h][c]{Reference}\hspace{\himg}
\makebox[\h][c]{Output}\vspace{0.3mm}
\\\
\includegraphics[width=\h]{figures/4.discussion/src1.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/4.discussion/ref1.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/4.discussion/out1.jpg}\vspace{-1mm}\\
\includegraphics[width=\h]{figures/4.discussion/src2.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/4.discussion/ref2.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/4.discussion/out2.jpg}\vspace{-1mm}\\
\includegraphics[width=\h]{figures/4.discussion/src3.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/4.discussion/ref3.jpg}\hspace{\himg}
\includegraphics[width=\h]{figures/4.discussion/out3.jpg}\vspace{0mm}
\caption{Reference-guided synthesis results on FFHQ with the model trained on CelebA-HQ. Despite the distribution gap between the two datasets, \stargan{} successfully extracts the style codes of the references and synthesizes faithful images.}
\label{fig:ffhq}
\vspace{-3mm}
\end{figure}
} 


\newcommand{\figafhqdataset}{
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/5.appendix/afhq_dataset.pdf}\\
\vspace{0mm}
\caption{Examples from our newly collected AFHQ dataset.}
\label{fig:afhq_dataset}
\vspace{-1mm}
\end{figure*}
}


\newcommand{\figrefcelebatwo}{
\begin{figure*}[t]
\centering
\begin{minipage}[c]{0.972\linewidth}
\includegraphics[width=1.0\linewidth]{figures/5.appendix/ref_celeba.pdf}\\
\vspace{-1mm}
\end{minipage}
\caption{Reference-guided image synthesis results on CelebA-HQ. 
The source and reference images in the first row and the first column are real images, while the rest are images generated by our proposed model, \stargan. Our model learns to transform a source image reflecting the style of a given reference image. High-level semantics such as hairstyle, makeup, beard and age are followed from the reference images, while the pose and identity of the source images are preserved. Note that the images in each column share a single identity with different styles, and those in each row share a style with different identities. 
}
\label{fig:refcelebatwo}
\vspace{-1mm}
\end{figure*}
}



\newcommand{\figrefafhq}{
\begin{figure*}[t]
\vspace{-5mm}
\centering
\begin{minipage}[c]{1.0\linewidth}
\includegraphics[width=1.0\linewidth]{figures/5.appendix/ref_afhq.pdf}\\
\vspace{-2mm}
\end{minipage}
\caption{Reference-guided image synthesis results on AFHQ. All images except the sources and references are generated by our proposed model, \stargan{}. High-level semantics such as hair are followed from the references, while the pose of the sources are preserved.}
\label{fig:refafhq}
\vspace{-1mm}
\end{figure*}
}
